Bayesian interpretation of Backus-Gilbert methods

The extraction of spectral densities from Euclidean correlators evaluated on the lattice is an important problem, as these quantities encode physical information on scattering amplitudes, finite-volume spectra, inclusive decay rates, and transport coefficients. In this contribution, we show that the Bayesian approach to this "inverse" problem, based on Gaussian processes, can be reformulated in a way that yields a solution equivalent, up to statistical uncertainties, to the one obtained in a Backus-Gilbert approach. After discussing this equivalence, we point out its implications for a reliable determination of spectral densities from lattice simulations.

==> Init.tex <==
%\pagestyle{headings}
%\textwidth=440pt
%\hoffset=-0.6truein
%%%%%%      %%%%%%      %%%%%%  
%%%%%%      Packages    %%%%%%  
%%%%%%      %%%%%%      %%%%%%  
\usepackage[utf8]{inputenc}
\usepackage {amsmath, amssymb, mathrsfs, graphics, setspace}
\usepackage{braket}
\usepackage{multirow}
\usepackage{amsthm}
\usepackage{bbold}
\usepackage{cancel}
\usepackage{slashed}
\usepackage{color}
\usepackage{bbm}
\usepackage{amsfonts}
\usepackage{ytableau}
\usepackage{graphicx}
\usepackage{cite}
\usepackage{nicefrac}
\usepackage[]{authblk}
\setlength{\affilsep}{3em}
\usepackage{setspace}
\usepackage{placeins}
\setstretch{1.02}
\usepackage{abstract}
\renewcommand{\abstractname}{}    % clear the title
\renewcommand{\absnamepos}{empty} % originally center
\pagestyle{myheadings}

%   some sectioning
\renewcommand{\thesection}{\Roman{section}}
\renewcommand{\thesubsection}{\thesection.\Roman{subsection}}
\usepackage{titlesec}
\titleformat*{\section}{\fontsize{10}{12}\bfseries\filcenter\MakeUppercase}
\titleformat*{\subsection}{\fontsize{9}{11}\bfseries\filcenter\MakeUppercase}
\titleformat*{\subsubsection}{\fontsize{8}{10}\bfseries\filcenter\MakeUppercase}
\titleformat*{\paragraph}{\fontsize{8}{10}\bfseries\filcenter\MakeUppercase}
\titleformat*{\subparagraph}{\fontsize{8}{10}\bfseries\filcenter\MakeUppercase}


\newcommand*{\email}[1]{%
    \normalsize\href{mailto:#1}{#1}\par
    }

%   %
\usepackage[linktocpage=true]{hyperref}
\usepackage{xcolor}
\hypersetup{
    colorlinks,
    linkcolor={blue!90!black},
    citecolor={blue!90!black},
    urlcolor={blue!90!black}
}
\iffalse
\hypersetup{
    colorlinks=true,
    linkcolor=black,
    filecolor=black,   
    citecolor=black,
    urlcolor=black,
    pdftitle={ },
    pdfpagemode=FullScreen,
    }
\fi
%%%%%%      %%%%%%      %%%%%%  
%%%%%%      Commands    %%%%%%  
%%%%%%      %%%%%%      %%%%%%  
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{thcheck}[theorem]{}
%Misc
\newcommand{\Op}{\mathcal{O}}
\newcommand{\idd}{\mathbb{1}}
\newcommand{\p}{^{\prime}}
\newcommand{\at}{\bigg\rvert}
\newcommand{\vet}{\boldsymbol}
\newcommand{\oneh}{\frac{1}{2}}
\newcommand{\de}{\partial}
\newcommand{\Lagr}{\mathcal{L}}
\newcommand{\Intrealpos}{\int_{0}^{\infty}}
\newcommand{\Intreal}{\int_{-\infty}^{\infty}}
\newcommand{\Intzerone}{\int_0^1}
\newcommand{\T}{\mathcal{T}}
\newcommand{\smatrix}{\begin{pmatrix}}
\newcommand{\cmatrix}{\end{pmatrix}}
\newcommand{\De}{\nabla}
\newcommand{\da}{^\dagger}
\DeclareMathOperator{\Tr}{Tr}
%Parentesi
\newcommand{\lr}{\left(}
\newcommand{\rr}{\right)}
\newcommand{\lcurl}{\left \{ }
\newcommand{\rcurl}{ \right\}}
%Mat elements
\newcommand{\matel}[3]{#1_{{#2}}^{\phantom{{#2}}{#3}}}
\newcommand{\matelc}[3]{#1^{{#2}}_{\phantom{{#2}}{#3}}}

\DeclareMathOperator{\ide}{\mathbbm{1}}


